Flexible Semantic-Aware Resource Allocation: Serving More Users Through Similarity Range Constraints

Semantic communication (SemCom) aims to enhance the resource efficiency of next-generation networks by transmitting the underlying meaning of messages, focusing on information relevant to the end user. Existing literature on SemCom primarily emphasizes learning the encoder and decoder through end-to-end deep learning frameworks, with the objective of minimizing a task-specific semantic loss function. Beyond its influence on the physical and application layer design, semantic variability across users in multi-user systems enables the design of resource allocation schemes that incorporate user-specific semantic requirements. To this end, \emph{a semantic-aware resource allocation} scheme is proposed with the objective of maximizing transmission and semantic reliability, ultimately increasing the number of users whose semantic requirements are met. The resulting resource allocation problem is a non-convex mixed-integer nonlinear program (MINLP), which is known to be NP-hard. To make the problem tractable, it is decomposed into a set of sub-problems, each of which is efficiently solved via geometric programming techniques. Finally, simulations demonstrate that the proposed method improves user satisfaction by up to $17.1\%$ compared to state of the art methods based on quality of experience-aware SemCom methods.

==> refs.tex <==
@Article{FresnoCL2022,
  author       =   "V. Fresno and A. Ariza-Casabona and V. Fresno and M. A. Marti",
  title 			 =   "{Information-Theoretic Compositional Distributional Semantics}",
  journal 		 = 	 "Computational Linguistics",
  year         = 	 "2022",
volume = "48",
number = "4"
}


@Article{HuttebrauckerArxiv2024,
  author       =   "T. Huttebraucker and M. Sana and E. C. Strinati",
  title 			 =   "{Latent Space Alignment for Semantic Channel Equalization }",
  journal 		 = 	 "arXiv preprint arXiv:2405.13511"
}
@Article{FontanariTEC2007,
  author       =   "J. F. Fontanari and L. I. Perlovsky",
  title 			 =   "{Evolving compositionality in evolutionary language games}",
  journal 		 = 	 "IEEE Transactions on Evolutionary Computation",
  year         = 	 "2007",
volume = "11",
number = "6",
pages = "758-769"
}
@Article{Carnap52,
  author       =   "R. Carnap and Y. Bar-Hillel",
  title 			 =   "{An Outline of a Theory of Semantic Information}",
  journal 		 = 	 "Technical Report No. 247",
  year         = 	 "1952",
  month        = 	 "Oct."
}

@inproceedings{GoerssSpringer2009,
  author       =   "P. G. Goerss and J. F. Jardine",
  title 			 =   "{Simplicial homotopy theory}",
  booktitle     		 = 	 "Springer Science & Business Media",
  year         = 	 "2009"
}
@inproceedings{BoydCUP2004,
  author       =   "S. Boyd and L. Vandenberghe",
  title 			 =   "{Convex Optimization}",
  booktitle     		 = 	 "Cambridge University Press",
  year         = 	 "2004",
}
@inproceedings{LewisWiley2008,
  author       =   "D. Lewis",
  title 			 =   "{Convention: A Philosophical
Study}",
  booktitle     		 = 	 "John Wiley & Sons",
  year         = 	 "2008",
}
@Article{SinhaArxiv2024,
  author       =   "S. Sinha and T. Premsri and P. Kordjamshidi",
  title 			 =   "{A Survey on Compositional Learning of AI Models: Theoretical and Experimental Practices}
",
  journal 		 = 	 "arXiv preprint arXiv:2406.08787",
  year         = 	 "2024"
}

@Article{HongLuoSPM2015,
  author       =   "M. Hong and M. Razaviyayn and Z. Q. Luo and J. S. Pang ",
  title 			 =   "{A Unified Algorithmic Framework for Block-Structured Optimization Involving Big Data: With Applications in Machine Learning and Signal Processing}
",
  journal 		 = 	 "IEEE Signal Processing Magazine",
  year         = 	 "2015",
  pages = "57-77",
  volume       = "33",
  number    = "1",
  month = "Dec."
}

@Article{XiaoArxiv2024,
  author       =   "X. Xiao and G. Liu and G. Gupta and D. Cao and S. Li and Y. Li and T. Fang and M.Cheng and P. Bogdan",
  title 			 =   "{Neuro-Inspired Information-Theoretic Hierarchical Perception for Multimodal Learning}
",
  journal 		 = 	 "arXiv preprint arXiv:2404.09403"
}

@Article{BeckArxiv2022,
  author       =   "F. A. Gers and J. Schmidhuber and F. Cummins",
  title 			 =   "{Learning to Forget: Continual Prediction with LSTM}
",
  journal 		 = 	 "Neural Computation",
  year         = 	 "2000",
  pages = "2451-2471",
  volume       = "12",
  number    = "10"
}

@inproceedings{VaswaniNIPS2017,
  author       =   "A. Vaswani and N. Shazeer and N. Parmar and J. Uszkoreit and L. Jones and A. N. Gomez and L. Kaiser and I. Polosukhin",
  title 			 =   "{Attention is All You Need}",
  booktitle 		 = 	 "in Proceedings of 
  31st Conference on Advances in Neural Information Processing Systems ",
  year         = 	 "2017",
  month        = "Dec.",
}
. 2015. .  . 

@inproceedings{PawlickWEIS2015,
  author       =   "J. Pawlick and Q. Zhu",
  title 			 =   "{Deception by Design: Evidence-Based Signaling Games for Network Defense}",
  booktitle     		 = 	 "Proceedings of the Workshop on the Economics of Inform. Security and Privacy, available at http://arxiv.org/
abs/1503.05458",
  year         = 	 "2015",
  address        = "Delft, The Netherlands",
  month = "Jun."
}

@Article{RiegelLNN2020,
  author       =   "R. Riegel and others",
  title 			 =   "{Logical Neural Networks}
",
  journal 		 = 	 "{arXiv:2006.13155 [cs]}",
  year         = 	 "2020",
  month       = "Jun.",
}
@Article{GoldfieldJSAC2020,
  author       =   "Z. Goldfield and Y. Polyanskiy",
  title 			 =   "{The Information Bottleneck Problem and its Applications in Machine Learning}
",
  journal 		 = 	 "IEEE Journal on Selected Areas in Information Theory",
  year         = 	 "2020",
  volume       = "1",
  number       = "1",
  month       = "Apr.",
  pages = "19-38"
}
@Article{BeckArxiv2022,
  author       =   "E. Beck and C. Bockelmann and A. Dekorsy",
  title 			 =   "{Semantic Communication: An Information Bottleneck View}
",
  journal 		 = 	 "arXiv preprint arXiv:2204.13366",
  year         = 	 "2022",
  month       = "Apr.",
}
@inproceedings{ZaslavskySCiL2021,
  author       =   "N. Zaslavsky and J. Hu and R. P. Levy",
  title 			 =   "{A Rate–Distortion View of Human Pragmatic Reasoning}",
  booktitle 		 = 	 "Proceedings of the Society for Computation in Linguistics (SCiL) ",
  year         = 	 "2021",
  pages        = "347–348",
}
@inproceedings{BordesNIPS2013,
  author       =   "A. Bordes and N. Usunier and A. Gari\'a-Dur\'an and J. Weston",
  title 			 =   "{Translating Embeddings for Modeling
Multi-relational Data}",
  booktitle 		 = 	 "In Advances in Neural Information
Processing Systems",
  year         = 	 "2013",
  pages        = "2787–2795",
}
@Article{UAM00,
  author       =   "M. K. Abdel-Aziz and S. Samarakoon and M. Bennis and W. Saad",
  title 			 =   "{Ultra-Reliable and Low-Latency Vehicular Communication: An Active Learning Approach}",
  journal 		 = 	 "IEEE Communications Letters",
  year         = 	 "2019",
  pages        = "367-370",
  volume       = "24",
  number       = "2"
}

@Article{LiangArxiv2022,
  author       =   "J. Liang and Y. Xiao and Y. Li and G. Shi and M. Bennis",
  title 			 =   "{Life-long Learning for Reasoning-based Semantic Communication}",
  journal 		 = 	 "arXiv preprint arXiv:2202.01952",
  year         = 	 "2022"
}
@inproceedings{BengioNeurIPS2021,
  author       =   "E. Bengio and M. Jain and M. Korablyov and
D. Precup and Y. Bengio.",
  title 			 =   "{Flow Network based
Generative Models for Non-Iterative Diverse Candidate
Generation}",
  booktitle 		 = 	 " Neural Information Processing Systems",
  year         = 	 "2021",
  month       = "Dec.",
}


@Article{BradleyMatematica2022,
  author       =   "T. D. Bradley and J. Terilla and Y. Vlassopulos",
  title 			 =   "{An Enriched Category Theory of Language: From Syntax to Semantics}
",
  journal 		 = 	 "La Matematica",
  year         = 	 "2022",
  pages = "1-30",
  month = "Mar."
}
@Article{FongArxiv2018,
  author       =   "B. Fong and D. I. Spivak",
  title 			 =   "{Seven Sketches in Compositionality: An Invitation to Applied
Category Theory}
",
  journal 		 = 	 "arXiv preprint arXiv:1803.05316",
  year         = 	 "2018",
  month = "Oct."
}
@inproceedings{CarlssonAMCSS,
  author       =   "E. Carlsson and
D. Dubhashi",
  title 			 =   "{Pragmatic Reasoning in Structured Signaling Games}
",
  booktitle 		 = 	 "Proceedings of the Annual Meeting of the Cognitive Science
Society",
  year         = 	 "2022",
  volume       = "44",
}
@Article{DeleuArxiv2022,
  author       =   "T. Deleu and others",
  title 			 =   "{Bayesian Structure Learning with Generative Flow Networks}
",
  journal 		 = 	 "arXiv preprint arXiv:2202.13903",
  year         = 	 "2022",
  month       = "Feb.",
}

@Article{LindleyAMS1956,
  author       =   "D. V. Lindley",
  title 			 =   "{On a Measure of the Information Provided by an Experiment}
",
  journal 		 = 	 "The Annals of Mathematical Statistics",
  year         = 	 "1956",
  month       = "Jul.",
  volume = "27",
  number = "4",
  pages = "986-1005"
}
@Article{SeoMehdiArxiv2022,
  author       =   "S. Seo and 
J. Park and S-W Ko and J. Choi and M. Bennis, and S-L Kim",
  title 			 =   "{Towards Semantic Communication Protocols:
A Probabilistic Logic Perspective}
",
  journal 		 = 	 "arXiv:2207.03920v1",
  year         = 	 "2022",
  month       = "Jul.",
}


@Article{PopovskiJIIS2020,
  author       =   "P. Popovski and O. Simeone and F. Boccardi and D. G{\"u}nd{\"u}z and O. Sahin",
  title 			 =   "{Semantic-Effectiveness Filtering and Control for Post-5G Wireless Connectivity
}",
  journal 		 = 	 "Journal of the Indian Institute of Science",
  year         = 	 "2020",
  volume        = "100",
  number        = "2",
  pages        = "435-443",
  month       = "Apr.",
}
@Article{CarlosSantana2014,
  author       =   "C. Santana",
  title 			 =   "{Ambiguity in Cooperative Signaling
}",
  journal 		 = 	 "Philosophy of Science,The University of Chicago Press on behalf of the Philosophy of Science
Association",
  year         = 	 "2014",
  volume        = "81",
  number        = "3",
  pages        = "398-422",
  month       = "Jul.",
}
@Article{XieJSAC2022,
  author       =   "H. Xie and Z. Qin and X. Tao and K. B. Letaief",
  title 			 =   "{Task-Oriented Multi-User Semantic
Communications
}",
  journal 		 = 	 "IEEE Journal on Selected Areas in Communications.",
  year         = 	 "2022",
  month       = "Jul.",
}

@Article{JagerGEB2011,
  author       =   "G. J\'{a}ger and L. P. Metzger and F. Riedel",
  title 			 =   "{Voronoi Languages: Equilibria in Cheap-talk Games with High-Dimensional Types and Few Signals
}",
  journal 		 = 	 "Games and Economic Behavior",
  volume       = "73",
  number       = "2",
  year         = 	 "2011",
  pages = "517--537",
  month       = "Nov.",
}

@inproceedings{FinnICML2017,
  author       =   "C. Finn and P. Abbeel and S. Levine",
  title 			 =   "{Model-agnostic Meta-learning for Fast Adaptation of Deep Networks.}",
  booktitle 		 = 	 " In International conference on machine learning",
  year         = 	 "2017",
  pages  = "1126-1135",
  address       = "Sydney, Australia",
}
@inproceedings{CoverThomas1991,
  author       =   "T. M. Cover and J. A. Thomas",
  title 			 =   "{Elements of Information Theory}",
  booktitle 		 = 	 "Wiley",
  year         = 	 "1991",
}
@inproceedings{ZhangBengio2022,
  author       =   "D. Zhang  and N. Malkin and Z. Liu and A. Volokhova and A. Courville and Y. Bengio",
  title 			 =   "{Generative Flow Networks for Discrete Probabilistic Modeling}",
  booktitle 		 = 	 " Proceedings of the 39 th International Conference on Machine
Learning",
  year         = 	 "2022",
  address       = "Maryland, USA",
  month = "Jul."
}
@Article{ZaslavskyArxiv2020,
  author       =   "N. Zaslavsky and H. Jennifer and R. P. Levy",
  title 			 =   "{A Rate-Distortion View of Human Pragmatic Reasoning.}
",
  journal 		 = 	 "arXiv preprint arXiv:2005.06641",
  year         = 	 "2020",
  month       = "May",
}
@inproceedings{BrownNIPS2020,
  author       =   "T. Brown and others",
  title 			 =   "{Language Models are Few-Shot Learners
}",
  booktitle 		 = 	 "Advances in Neural Information Processing Systems 33 (NeurIPS)",
  year         = 	 "2020",
  address       = "Vancouver, Canada",
  month = "Dec."
}
@inproceedings{RaedtIJCAI2020,
  author       =   "L. D. Raedt and
 S. Duman\v ci\'c
and Robin Manhaeve
and Giuseppe Marra",
  title 			 =   "{From Statistical Relational to Neural-Symbolic Artificial Intelligence}",
  booktitle 		 = 	 "Proceedings of the Twenty-Ninth International Joint Conference on Artificial Intelligence (IJCAI-20)
Survey Track",
  year         = 	 "2020",
  address       = "Yokohama, Japan",
}
@inproceedings{KahnemanNewYork2011,
  author       =   "D. Kahneman,
D. Precup, and Y. Bengio",
  title 			 =   "{Thinking, Fast and Slow}",
  booktitle 		 = 	 " Farrar, Straus and Giroux",
  year         = 	 "2011",
  address       = "New York",
}
@Article{GarcezArxiv2020,
  author       =   "A. A. Garcez and L. C. Lamb",
  title 			 =   "{Neurosymbolic AI: the 3rd Wave}",
  journal 		 = 	 "arXiv preprint arXiv:2012.05876",
  year         = 	 "2020",
  month   = "Dec."
  }
 
  @Article{ShannonBSTJ1948,
  author       =   "C. E. Shannon",
  title 			 =   "{A Mathematical Theory of Communication}",
  journal 		 = 	 "in The Bell System Technical Journal",
  year         = 	 "1948",
  volume       = "27",
  number       = "3",
  pages        ="379-423",
  month        = "Jul."
}

@Article{TOSheaTCN2017,
  author       =   "T. O'Shea and J. Hoydis",
  title 			 =   "{An Introduction to Deep Learning for the Physical Layer
}",
  journal 		 = 	 "IEEE Transactions on Cognitive Communications and Networking",
  volume = "3",
  number = "4",
  pages = "563-575",
  year         = 	 "2017"
  }

@Article{RatliffTAC2016,
  author       =   "L. J. Ratliff and S. A. Burden and S. S. Shastry",
  title 			 =   "{On the Characterization of Local Nash Equilibria in Continuous Games
}",
  journal 		 = 	 "IEEE Transactions on Automatic Control",
  year         = 	 "2016",
  volume = "61",
  number = "8",
  pages = "2301-2307",
  month = "Jun."
  }
@Article{FacchineiAOR2010,
  author       =   "F. Facchinei and C. Kanzow",
  title 			 =   "{Generalized Nash Equilibrium Problems
}",
  journal 		 = 	 "Annals of Operations Research",
  year         = 	 "2010",
  volume = "175",
  number = "1",
  pages = "177-2011",
  month = "Sep."
  }
@Article{Smolenskyarxiv2022,
  author       =   "P. Smolensky and R. T. McCoy and R. Fernandez and M. Goldrick, J. Gao",
  title 			 =   "{Neurocompositional computing: From the Central Paradox of Cognition to a new generation of AI systems
}",
  journal 		 = 	 "arXiv preprint arXiv:2205.01128",
  year         = 	 "2022"
  }


@Article{WeiChainReasonArxiv2022,
  author       =   "J. Wei and X. Wang and D. Schuurmans and M. Bosma and E. Chi and Q. Le and D. Zhou",
  title 			 =   "{Chain of Thought Prompting Elicits Reasoning in Large Language Models
}",
  journal 		 = 	 "arXiv preprint arXiv:2201.11903",
  year         = 	 "2022",
  month = "Oct."
  }
@inproceedings{FudenbergCambridge1991,
  author       =   "D. Fudenberg and J. Tirole",
  title 			 =   "{Game Theory}",
  booktitle 		 = 	 "Cambridge, MA: MIT Press",
  year         = 	 "1991",
}
@inproceedings{DasICCCV2017,
  author       =   "A. Das and S. Kottur and J. M.F. Moura and S. Lee and D. Batra",
  title 			 =   "{Learning Cooperative Visual Dialog Agents with Deep Reinforcement Learning}",
  booktitle 		 = 	 "IEEE International Conference on Computer Vision",
  year         = 	 "2017",
}
@inproceedings{MotaHoydis2021,
  author       =   "M. P. Mota and A. Valcarce and J.-M. Gorce
and J. Hoydis",
  title 			 =   "{The Emergence of Wireless MAC Protocols with
Multi-Agent Reinforcement Learning}",
  booktitle 		 = 	 "arXiv:2108.07144. [Online]. Available: https://arxiv.org/abs/2108.07144",
  year         = 	 "2021",
}
@inproceedings{KotturEMNLP2017,
  author       =   "S. Kottur and J. F. Moura and S. Lee and D. Batra",
  title 			 =   "{Natural Language Does Not Emerge 'Naturally' in Multi-Agent Dialog}",
  booktitle 		 = 	 "Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing",
  year         = 	 "2017",
  pages = "2962-2967",
  address       = "Copenhagen, Denmark",
  month     = "Sep."
}
@inproceedings{MerluzziEuCNC2022,
  author       =   "M. Merluzzi and M. C. Filippou and L. G. Baltar and Calvanese Strinati, Emilio",
  title 			 =   "{Effective Goal-oriented 6G Communications: the Energy-aware Edge Inferencing Case}",
  booktitle 		 = 	 " IEEE EuCNC and 6G Summit",
  year         = 	 "2022",
  address       = "Grenoble, France",
  month     = "Jun."
}


@Article{KountourisCommMag2021,
  author       =   "M. Kountouris and N. Pappas",
  title 			 =   "Semantics-empowered communication for networked intelligent systems",
  journal 		 = 	 "IEEE Communications Magazine",
  year         = 	 "202",
  pages        = "96-102",
  volume       = "59",
  number       = "6",
  month = "Jun."
}
@Article{RISMY03,
  author       =   "M. K. Abdel-Aziz and S. Samarakoon and C. F. Liu and M. Bennis and W. Saad",
  title 			 =   "Optimized age of information tail for ultra-reliable low-latency communications in vehicular networks",
  journal 		 = 	 "IEEE Transactions on Communications",
  year         = 	 "2019",
  pages        = "1911-1924",
  volume       = "68",
  number       = "3"
}

@inproceedings{KingmaICLR2013,
  author       =   "D. P. Kingma and M. Welling",
  title 			 =   "{Auto-Encoding Variational Bayes}",
  booktitle 		 = 	 " In The 2nd International Conference
on Learning Representations (ICLR)",
  year         = 	 "2013",
  month        = 	 "May"
}
@inproceedings{HigginsICLR2017,
  author       =   "I. Higgins and others",
  title 			 =   "{\textbeta-VAE: Learning Basic Visual Concepts with a
Constrained Variational Framework}",
  booktitle 		 = 	 "ICLR",
  year         = 	 "2017",
  month        = 	 "Apr."
}
@Article{Badreddine2022,
  author       =   "S. Badreddine and A. D. A. Garcez and L. Serafini and M. Spranger",
  title 			 =   "{Logic Tensor Networks}",
  journal 		 = 	 "Artificial Intelligence",
  year         = 	 "2022",
  volume       = "303",
  month        = 	 "Oct."
}
@inproceedings{CarnapCUP1962,
  author       =   "R. Carnap",
  title 			 =   "{Logical Foundations of Probability}",
  booktitle 		 = 	 "Chicago: University of Chicago press",
  year         = 	 "1962",
  volume       = "2",
  month        = 	 "Dec."
}
@inproceedings{HiriartSpringer1985,
  author       =   "J. B Hiriart-Urruty",
  title 			 =   "{Generalized Differentiability, Duality and Optimization for Problems
Dealing with Differences of Convex Functions}",
  booktitle 		 = 	 " Convexity and Duality in Optimization, Springer",
  year         = 	 "1985",
}

@Article{MiuccioArxiv2022,
  author       =   "L. Miuccio and S. Riolo and S. Samarakoony and D. Panno and M. Bennis",
  title 			 =   "{Learning Generalized Wireless MAC Communication Protocols via Abstraction}",
  journal 		 = 	 "arXiv preprint arXiv:2206.06331.",
  year         = 	 "2022",
  month        = 	 "Jun."
}
@Article{HoffmanJMLR2013,
  author       =   "M. D. Hoffman and D. M. Blei and C. Wong and J. Paisley",
  title 			 =   "{Stochastic Variational Inference}",
  journal 		 = 	 "Journal of Machine Learning Research",
  year         = 	 "2013",
  month        = 	 "May",
  pages = "1303-1347",
  volume = "14"
}

@Article{AhujaICML2020,
  author       =   "K. Ahuja and K. Shanmugam and K. Varshney and A. Dhurandhar",
  title 			 =   "{Invariant risk minimization games
}",
  journal 		 = 	 "In International Conference on Machine Learning",
  year         = 	 "2020",
  volume = "31",
  month = "November",
  pages = "145-155"
}
@Article{MagliacaneNIPS2018,
  author       =   "S. Magliacane and T. V. Ommen and T. Claassen and S. Bongers and P. Versteeg and J. M. Mooij",
  title 			 =   "{Domain adaptation by using causal inference to predict invariant conditional distributions
}",
  journal 		 = 	 "Advances in neural information processing systems",
  year         = 	 "2018",
  volume = "31",
  pages = "7399-7407"
}
@Article{BLiAAAI2022,
  author       =   "B. Li and Y. Shen and Y. Wang and W. Zhu and D. Li and K. Keutzer and H. Zhao",
  title 			 =   "{Invariant information bottleneck for domain generalization
}",
  journal 		 = 	 "In Proceedings of the AAAI Conference on Artificial Intelligence",
  year         = 	 "2022",
  volume = "36",
  number = "07",
  pages = "7399-7407"
}
@Article{TomarArxiv2021,
  author       =   "M. Tomar and A. Zhang and R. Calendra and M. E. Taylor and J. Pineau",
  title 			 =   "{Model-Invariant State Abstractions for Model-Based
Reinforcement Learning
}",
  journal 		 = 	 "arXiv preprint arXiv:2102.09850",
  year         = 	 "2021"
}
@Article{ArumugamNIPS2021,
  author       =   "D. Arumugam and B. V. Roy",
  title 			 =   "{The value of information when deciding what to learn}",
  journal 		 = 	 "Advances in Neural Information Processing Systems",
  year         = 	 "2021",
  volume = "34",
  pages = "9816-9827",
  month        = 	 "May"
}
@Article{Fagin2021,
  author       =   "R. Fagin and R. Riegel and A. Gray",
  title 			 =   "{Foundations of Reasoning with Uncertainty via Real-valued Logics}",
  journal 		 = 	 "arXiv preprint arXiv:2008.02429",
  year         = 	 "2021",
  month        = 	 "May"
}
@Article{Socher2013,
  author       =   "R. Socher and D. Chen and C. D. Manning and A. Y. Ng",
  title 			 =   "Reasoning with neural tensor networks for knowledge base completion.",
  journal 		 = 	 "Advances in Neural Information Processing Systems",
  year         = 	 "2013"
}

@Article{GunduzJSAC2022,
  author       =   "D. G{\"u}nd{\"u}z and others",
  title 			 =   "{Beyond Transmitting Bits: Context, Semantics, and
Task-Oriented Communications}",
  journal 		 = 	 "In: arXiv:2207.09353v1",
  year         = 	 "2022",
  month = "Jul.",
}
@Article{Shannon1948,
  author       =   "C. E. Shannon",
  title 			 =   "A Mathematical Theory of Communication",
  journal 		 = 	 "The Bell System Technical Journal",
  year         = 	 "1948",
  volume      = "27",
  number      = "3",
  pages       = "379-423",
}


  @inproceedings{Bengio2019,
  title={From System 1 Deep Learning to System 2 Deep Learning},
  author={Y. Bengio},
  booktitle={Keynote at NeurIPS},
  year={2019}
}
@inproceedings{ThomasGC2022,
  author       =   "C. K. Thomas and W. Saad",
  title        =   "{Neuro-Symbolic Artificial Intelligence (AI) for Intent based Semantic Communication}", 
  booktitle      = 	 "Proceedings of IEEE Global Communications Conference (GLOBECOM)",
  year         = 	 "2022",
  month        = "Dec",
}
@inproceedings{ChoiArxiv2022,
  author       =   "J. Choi and S. W. Loke and J. Park",
  title        =   "{A Unified View on Semantic Information and
Communication: A Probabilistic Logic Approach}", 
  booktitle      = 	 "In: arXiv preprint arXiv:2201.05936",
  year         = 	 "2022"
}
@inproceedings{Guha2015,
  author       =   "R. V. Guha",
  title        =   "{Towards A Model Theory for Distributed Representations}", 
  booktitle      = 	 "In: AAAI Spring Symposium",
  year         = 	 "2015"
}

@inproceedings{RibeiroISR2004,
  author       =   "M. I. Ribeiro",
  title        =   "{Kalman and Extended Kalman Filters: Concept, Derivation and Properties}", 
  booktitle      = 	 "Institute for Systems and Robotics",
  year         = 	 "2004"
}
@inproceedings{DavidNIPS2018,
  author       =   "D. Ha and J. Schmidhuber",
  title        =   "{Recurrent World Models Facilitate Policy Evolution}", 
  booktitle      = 	 "Advances in Neural Information Processing Systems 31 (NeurIPS)",
  year         = 	 "2018"
}
@inproceedings{PetersMIT2017,
  author       =   "J. Peters, D. Janzing, and B. Schölkopf",
  title        =   "{Elements of Causal Inference - Foundations and Learning
Algorithms}", 
  booktitle      = 	 "MIT Press, Cambridge, MA, USA",
  year         = 	 "2017"
}

@inproceedings{ChaccourICC2022,
  author       =   "C. Chaccour, W. Saad, O. Semiari and M. Bennis, and P. Popovski",
  title        =   "{Joint Sensing and Communication for Situational Awareness in Wireless THz Systems}", 
  booktitle      = 	 "Proceedings of IEEE International Conference on Communications (ICC)",
  year         = 	 "2022",
  month        = "May"
}



@Article{YangAccess2018,
  author       =   "X. Yang and Z. Chen and K. Li and Y. Sun and N. Liu and W. Xie and Y. Zhao",
  title 			 =   "{Communication-Constrained Mobile Edge Computing
Systems for Wireless Virtual Reality: Scheduling and Tradeoff}",
  journal 		 = 	 "IEEE
Access",
  volume         = 	 "6",
  pages = "16665-16677",
  year = "2018"
}
@Article{ChenTCOM2018,
  author       =   "M. Chen, W. Saad, and C. Yin",
  title 			 =   "{Virtual Reality over Wireless Networks:
Quality-of-service Model and Learning-based Resource Management}",
  journal 		 = 	 "IEEE Trans. on Commun.",
  volume         = 	 "66",
  number  = "11",
  pages = "5621–5635",
  month = "Nov.",
  year = "2018"
}

@Article{HuiqiangJSAC2022,
  author       =   "X. Huiqiang, Z. Qin, X. Tao, and K. B. Letaief",
  title 			 =   "{Task-oriented Multi-user Semantic Communications}",
  journal 		 = 	 "IEEE Journal on Selected Areas in Communications",
  volume         = 	 "40",
  number  = "09",
  pages = "2584-2597",
  month = "Nov.",
  year = "2022"
}

@Article{PriebeTWC2013,
  author       =   "S. Priebe and T. Kurner",
  title 			 =   "{Stochastic Modeling of THz Indoor Radio Channels}",
  journal 		 = 	 " IEEE Transac Wireless Commun.",
  volume         = 	 "12",
  number  = "09",
  pages = "4445–4455",
  month = "Sep.",
  year = "2013"
}

@Article{MashhadiTWC2010,
  author       =   "M. B. Mashhadi and D. G{\"u}nd{\"u}z",
  title 			 =   "{Deep Learning-based Pilot Design and Channel Estimation for MIMO-OFDM Systems}",
  journal 		 = 	 "IEEE Transactions on Wireless Communications",
  year = "2010",
  volume = "20",
  number = "10",
  pages = "6315-6328"
}

@Article{Al-TanDaiJSAC2021,
  author       =   "J. Tan and L. Dai",
  title 			 =   "{Wideband Beam Tracking in THz Massive
MIMO Systems}",
  journal 		 = 	 "IEEE Journal on Selected Areas in Communications",
  volume         = 	 "39",
  number  = "6",
  pages = "1693-1710",
  month = "Jun.",
  year = "2021"
}
@Article{Al-NaffouriTSP2007,
  author       =   "T. Y. Al-Naffouri",
  title 			 =   "{An EM-based Forward-Backward Kalman Filter for the Estimation of Time-variant Channels in OFDM}",
  journal 		 = 	 "IEEE Transactions on Signal Processing",
  volume         = 	 "55",
  number  = "7",
  pages = "3924-3930",
  month = "Jun.",
  year = "2007"
}
@Article{GiannakisTIT2011,
  author       =   "S. J. Kim and G. B. Giannakis",
  title 			 =   "{Optimal Resource Allocation for MIMO Ad hoc Cognitive Radio Networks}",
  journal 		 = 	 "IEEE Transactions on Information Theory",
  volume         = 	 "57",
  number  = "5",
  pages = "3117-3131",
  month = "Apr.",
  year = "2011"
}
@Article{AnsonArxiv2022,
  author       =   "L. Anson and B. Schölkopf and I. Posner",
  title 			 =   "{Variational Causal Dynamics: Discovering Modular World Models from Interventions}",
  journal 		 = 	 "arXiv preprint arXiv:2206.11131",
  year = "2022"
}

@Article{AnsonArxiv2022,
  author       =   "L. Anson and B. Schölkopf and I. Posner",
  title 			 =   "{Variational Causal Dynamics: Discovering Modular World Models from Interventions}",
  journal 		 = 	 "arXiv preprint arXiv:2206.11131",
  year = "2022"
}

@Article{MoerlandArxiv2020,
  author       =   "T. M. Moerland and J. Broekens and C. M. Jonker",
  title 			 =   "{Model-based Reinforcement Learning: A Survey}",
  journal 		 = 	 "arXiv preprint arXiv:2006.16712",
  year = "2020"
}

@Article{PetersArxiv2015,
  author       =   "J. Peters and N. Meinshausen",
  title 			 =   "{Causal Inference using Invariant Prediction: Identification and Confidence Intervals.}",
  journal 		 = 	 "arXiv preprint 	arXiv:1501.01332",
  year = "2015"
}
 
@Article{ArjovskyCoRR2015,
  author       =   "M. Arjovsky and L. Bottou and I. Gulrajani and D. Lopez-Paz",
  title 			 =   "{Invariant Risk Minimization}",
  journal 		 = 	 "CoRR, abs/1907.02893",
  year = "2019"
}

@Article{MohamedNIPS2015,
  author       =   "S. Mohamed and D. J. Rezende",
  title 			 =   "{Variational information maximisation for intrinsically motivated reinforcement learning}",
  journal 		 = 	 "Advances in neural information processing systems",
  volume = "28",
  year = "2015"
}

@Article{Kipfarxiv2019,
  author       =   "T. Kipf and E. Van der Pol and M. Welling",
  title 			 =   "{Contrastive learning of structured world models}",
  journal 		 = 	 "arXiv preprint arXiv:1911.12247",
  year = "2019"
}

@Article{WellsJPSP1989,
  author       =   "G. L. Wells and I. Gavanski",
  title 			 =   "{Mental simulation of causality. Journal of personality and social psychology}",
  journal 		 = 	 "Journal of personality and social psychology",
  volume = "56",
  number = "2",
  year = "1989"
}

@Article{PoudelArxiv2022,
  author       =   "R. P. Poudel and H. Pandya and R. Cipolla",
  title 			 =   "{Contrastive Unsupervised Learning of World Model with Invariant Causal Features}",
  journal 		 = 	 "arXiv preprint arXiv:2209.14932",
  year = "2022"
}

@Article{MadumalAAAI2020,
  author       =   "P. Madumal and T. Miller and L. Sonenberg and F. Vetere",
  title 			 =   "{Explainable reinforcement learning through a causal lens}",
  journal 		 = 	 "Proceedings of the AAAI conference on artificial intelligence",
  volume = "34",
  number = "3",
  pages = "2493-2500",
  month = "April",
  year = "2020"
}
@Article{MillerKER2021,
  author       =   "T. Miller",
  title 			 =   "{Contrastive explanation: A structural-model approach}",
  journal 		 = 	 "The Knowledge Engineering Review",
  volume = "36",
  year = "2021"
}
@Article{ChandakICL2020,
  author       =   "S. Chandak and F. Chiariotti and P. Popovski",
  title 			 =   "{Hidden Markov Model-Based Encoding for Time-Correlated IoT Sources}",
  journal 		 = 	 "IEEE Communications Letters",
  volume = "25",
  number = "5",
  pages = "1463-1467",
  year = "2020"
}
@Article{EppeAI2018,
  author       =   "M. Eppe and E. Maclean, R. Confalonieri and O. Kutz,
M. Schorlemmer and E. Plaza and K. Kühnberger ",
  title 			 =   "{A computational framework for conceptual blending}",
  journal 		 = 	 "Nature Machine Intelligence",
  volume = "4",
  number = "1",
  pages = "11-20",
  year = "2018"
}
@Article{EppeNMI2022,
  author       =   "M. Eppe and C. Gumbsch and M. Kerzel and P. D. Nguyen and M. V. Butz and S. Wermter",
  title 			 =   "{Intelligent Problem-solving as Integrated Hierarchical Reinforcement Learning}",
  journal 		 = 	 "Nature Machine Intelligence",
  volume = "4",
  number = "1",
  pages = "11-20",
  year = "2022"
}

@Article{AlemiArxiv2016,
  author       =   "A. A. Alemi and I. Fischer and J. V. Dillon and K. Murphy",
  title 			 =   "{Deep Variational Information Bottleneck}",
  journal 		 = 	 "arXiv preprint arXiv:1612.00410",
  year = "2016"
}
@Article{WarglienSynthese2013,
  author       =   "M. Warglien and P. G{\" a}rdenfors",
  title 			 =   "{Semantics, Conceptual Spaces, and the Meeting of Minds.}",
  journal 		 = 	 "Synthese",
  year = "2013",
  volume = "190",
  number = "12",
  pages = "2165-2193"
}
@inproceedings{YuanNeurIPS2019,
  author       =   "L. Yuan and Z. Fu and L. Zhou and K. Yang and S-C Zhu",
  title 			 =   "{Emergence of Theory of Mind Collaboration in
Multiagent Systems}",
  booktitle 		 = 	 "33rd Conference on Neural Information Processing Systems (NeurIPS)",
  year = "2019",
  month = "Dec.",
  address = "Vancouver, Canada"
}

@Article{EysenbachNIPS2021,
  author       =   "B. Eysenbach and R. R. Salakhutdinov and S. Levine",
  title 			 =   "{Robust Predictable Control}",
  journal 		 = 	 "Advances in Neural Information Processing Systems",
  year = "2021",
  volume = "34",
  pages = "27813-27825",
}
@Article{HafnerPMLR2019,
  author       =   "D. Hafner and T. Lillicrap and T. Fischer and T. Villegas D. Ha and H. Lee and J. Davidson",
  title 			 =   "{Learning Latent Dynamics
for Planning from Pixels}",
  journal 		 = 	 "Proceedings of the 36th International Conference on Machine Learning (PMLR)",
  year = "2019",
  volume = "97",
  month = "Jun."
}
@Article{ThomasArxiv2022,
  author       =   "C. K. Thomas and W. Saad",
  title 			 =   "{Neuro-Symbolic Causal Reasoning Meets Signaling Game for Emergent Semantic Communications}",
  journal 		 = 	 "arXiv preprint arXiv:2210.12040 ",
  year = "2022"
}
@inproceedings{SamarakoonSPAWC2021,
  author       =   "S. Samarakoon and J. Park and M. Bennis",
  title        =   "{Robust Reconfigurable iIntelligent Surfaces via Invariant Risk and Causal Representations}", 
  booktitle      = 	 "Proceedings of 22nd IEEE International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)",
  year         = 	 "2021"
}

@INPROCEEDINGS{Sana2022,
  author={M. Sana and E. C. Strinati },
  booktitle={Proceedings of IEEE 19th Annual Consumer Communications and Networking Conference (CCNC)}, 
  title={{Learning Semantics: An Opportunity for Effective 6G Communications}}, 
  year={2022},
  volume={},
  number={},
  pages={631-636},
  doi={10.1109/CCNC49033.2022.9700645}}

